An Optimization Framework for Power Infrastructure Planning

The ubiquitous expansion and transformation of the energy supply system involves large-scale power infrastructure construction projects. In the view of investments of more than a million dollars per kilometre, planning authorities aim to minimise the resistances posed by multiple stakeholders. Mathematical optimisation research offers efficient algorithms to compute globally optimal routes based on geographic input data. We propose a framework that utilizes a graph model where vertices represent possible locations of transmission towers, and edges are placed according to the feasible distance between neighbouring towers. In order to cope with the specific challenges arising in linear infrastructure layout, we first introduce a variant of the Bellman-Ford algorithm that efficiently computes the minimal-angle shortest path. Secondly, an iterative procedure is proposed that yields a locally optimal path at considerably lower memory requirements and runtime. Third, we discuss and analyse methods to output k diverse path alternatives. Experiments on real data show that compared to previous work, our approach reduces the resistances by more than 10% in feasible time, while at the same time offering much more flexibility and functionality. Our methods are demonstrated in a simple and intuitive graphical user interface, and an open-source package (LION) is available at https://pypi.org/project/lion-sp.

==> tables/backup_bl.tex <==
\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}                               & \textbf{Baseline} & 34.1  & 3595668   & 27.0 & 24.3  & 0.0    \\

\cellcolor[HTML]{F5F5F5}                                   & \multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{0.0}} & \textbf{Ours}     & 197.4 & 220339704 & 22.8 & 20.5  & 823.3  \\

\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}                               & \textbf{Baseline} & 35.6  & 3595668   & 25.4 & 25.4  & 0.0    \\

\cellcolor[HTML]{F5F5F5}                                   & \multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{0.1}} & \textbf{Ours}     & 196.8 & 220339704 & 7.7  & 20.8  & 943.5  \\

\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}                               & \textbf{Baseline} & 33.1  & 3595668   & 17.9 & 28.2  & 0.0    \\

\multirow{-6}{*}{\cellcolor[HTML]{F5F5F5}\textbf{austria}} & \multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{0.3}} & \textbf{Ours}     & 208.2 & 220339704 & 2.6  & 21.6  & 1413.8 \\

\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}                               & \textbf{Baseline} & 23.8  & 2205760   & 8.0  & 109.9 & 0.0    \\

\cellcolor[HTML]{F5F5F5}                                   & \multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{0.0}} & \textbf{Ours}     & 594.0 & 286284624 & 11.0 & 98.6  & 263.0  \\

\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}                               & \textbf{Baseline} & 21.9  & 2205760   & 9.6  & 118.4 & 0.0    \\

\cellcolor[HTML]{F5F5F5}                                   & \multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{0.1}} & \textbf{Ours}     & 588.5 & 286284624 & 2.7  & 101.5 & 482.5  \\

\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}                               & \textbf{Baseline} & 20.0  & 2205760   & 6.8  & 122.7 & 0.0    \\
\multirow{-6}{*}{\cellcolor[HTML]{F5F5F5}\textbf{belgium}} & \multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{0.3}} & \textbf{Ours}     & 583.4 & 286284624 & 1.2  & 105.4 & 498.0 


==> tables/backup_instances.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccccccc}
\textbf{Instance} & \textbf{\begin{tabular}[c]{@{}c@{}}Raster\\ width\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Raster\\ height\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Project region\\  (not forbidden)\end{tabular}} & \textbf{d\_min} & \textbf{d\_max} & \textbf{\begin{tabular}[c]{@{}c@{}}\#neigh-\\ bours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Estimated  \\ \#edges\end{tabular}} \\ \hline
\textbf{1}        & 1300                                                            & 739           & \begin{tabular}[c]{@{}c@{}}454 392 cells (81\%) \\ 45.4 km$^2$ \end{tabular}                                                                     & 15              & 25              & 632                                                               & \multicolumn{1}{r}{287 175 744}               \\
\textbf{2}        & 3078                                                            & 3724          & \begin{tabular}[c]{@{}c@{}} 1 498 585 (17\%) \\ 149.8 km$^2$ \end{tabular}                                                                     & 35              & 50              & 2002                                                              & 3 000 167 170                                                                 \\
\textbf{3}        & 3120                                                            & 2092       & \begin{tabular}[c]{@{}c@{}} 3 574 446 (57\%) \\ 357.4 km$^2$ \end{tabular}                                                                    & 15              & 25              & 632                                                               & 2 259 049 872                                                                              
\end{tabular}%
}
\caption{Instance properties, sizes and parameters: All numbers refer to a raster of 10 times 10 meters cells. The graph size is differs and depends on the size of the region, the forbidden areas and minimum and maximum distance between pylons.\todo{angle weight?}}
\label{tab:instances}
\end{table}

==> tables/baseline.tex <==
\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccl}
\multicolumn{1}{l}{\textbf{}}                              & \multicolumn{1}{l}{\textbf{}}             & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}} \textbf{Time} \\ \textbf{(seconds)} \end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\textbf{\#edges}\\ \textbf{in mio}\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}} \textbf{Angle} \\ \textbf{cost} \end{tabular}} & \multicolumn{1}{l}{\textbf{Resistance}} & \multicolumn{1}{l}{
\begin{tabular}[c]{@{}c@{}}\textbf{Avg. distance to} \\ \textbf{line-routing (in m)}\end{tabular}} &                      \\ \hline \\
\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}\textbf{line-routing} & \cellcolor[HTML]{F5F5F5}39.8                & \cellcolor[HTML]{F5F5F5}\textbf{2.2 }             & \cellcolor[HTML]{F5F5F5}9.9             & \cellcolor[HTML]{F5F5F5}110.6           & \cellcolor[HTML]{F5F5F5}0.0                                                        &                      \\
\multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{Inst. 1}} & \cellcolor[HTML]{F5F5F5}\textbf{Ours}     & 436.8                                       & 276.7                                    & \textbf{4.7}                                     & \textbf{97.9}                                    & 422.2                                                                                                                               & \multicolumn{1}{r}{} \\
\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}\textbf{line-routing} & \cellcolor[HTML]{F5F5F5}56.3                & \cellcolor[HTML]{F5F5F5}\textbf{3.5}              & \cellcolor[HTML]{F5F5F5}29.5            & \cellcolor[HTML]{F5F5F5}23.5            & \cellcolor[HTML]{F5F5F5}0.0                                                            &                      \\
\multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{Inst. 2}} & \cellcolor[HTML]{F5F5F5}\textbf{Ours}     & 155.9                                       & 138.1                                    & \textbf{15.8}                                    & \textbf{18.9}                                    & 743.7                                                                                                                             & \multicolumn{1}{r}{} \\
\cellcolor[HTML]{F5F5F5}                                   & \cellcolor[HTML]{F5F5F5}\textbf{line-routing} & \cellcolor[HTML]{F5F5F5}20.2                & \cellcolor[HTML]{F5F5F5}\textbf{1.4 }             & \cellcolor[HTML]{F5F5F5}15.5            & \cellcolor[HTML]{F5F5F5}13.7            & \cellcolor[HTML]{F5F5F5}0.0                                                                         &                      \\
\multirow{-2}{*}{\cellcolor[HTML]{F5F5F5}\textbf{Inst. 3}} & \cellcolor[HTML]{F5F5F5}\textbf{Ours}     & 337.3                                       & 178.3                                    & \textbf{11.2}                                    & \textbf{11.4 }                                   & 354.1                                                                                                                       & \multicolumn{1}{r}{} \\
\multicolumn{1}{l}{}                                       & \multicolumn{1}{l}{}                      & \multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                         & \multicolumn{1}{l}{}                    & \multicolumn{1}{l}{}                                                   & \multicolumn{1}{l}{}                                                   &                     
\end{tabular}%
}
\caption{Comparison of our graph modelling to the line-routing, where each cell is connected to its 8-neighborhood. The better result is marked bold in each case. Although our approach leads to much larger graphs, the optimal path can still be computed in minutes and in all cases leads to significantly lower angle and resistance costs. Also, the routes are substantially different, such that a local search around the computed route does not suffice to determine the optimal path.}
\label{tab:line-routing}
\end{table}
